Explicit feedback synthesis for nonlinear robust model predictive control driven by quasi-interpolation

We present QuIFS (Quasi-Interpolation driven Feedback Synthesis): an offline feedback synthesis algorithm for explicit nonlinear robust minmax model predictive control (MPC) problems with guaranteed quality of approximation. The underlying technique is driven by a particular type of grid-based quasi-interpolation scheme. The QuIFS algorithm departs drastically from conventional approximation algorithms that are employed in the MPC industry (in particular, it is neither based on multi-parametric programming tools and nor does it involve kernel methods), and the essence of its point of departure is encoded in the following challenge-answer approach: Given an error margin $\varepsilon>0$, compute in a single stroke a feasible feedback policy that is uniformly $\varepsilon$-close to the optimal MPC feedback policy for a given nonlinear system subjected to constraints and bounded uncertainties. Closed-loop stability and recursive feasibility under the approximate feedback policy are also established. We provide a library of numerical examples to illustrate our results.

==> Num_Ex_0.tex <==
\begin{example}\label{exmp:lmpc_0}
Consider the fourth-order linear dynamical system:
\begin{align}\label{eq:fourth_order_dyn_II}
    x_{t+1} = Ax_t + B u_t + w_t,
\end{align}
with the state and the actuation matrices:
\[A \Let \begin{pmatrix} 0.4035 & 0.3704 & 0.2935 & -0.7258 \\ -0.2114 & 0.6405 & -0.6717 & -0.0420 \\ 0.8368 & 0.0175 & -0.2806 & 0.3808 \\ -0.0724 & 0.6001 & 0.5552 & 0.4919 \end{pmatrix},\]
\[B \Let \begin{pmatrix} 1.6124 & 0.4086 & -1.4512 & -0.6761 \end{pmatrix}^{\top}.\]
Fix \(N=17\) and consider the robust optimal control problem:
\textcolor{blue}{\begin{equation}
	\label{eq:RMPC_fourth_order_II}
	\begin{aligned}
		&  \inf_{(\pi_t)_{t=0}^{\horizon-1}} \sup_{{W}} && \sum_{t=0}^{\horizon-1} \inprod{\dummyx_t}{Q\dummyx_t} + \inprod{\dummyu_t}{R\dummyu_t} \\
		& \sbjto && \begin{cases}
			 \text{the dynamics }\eqref{eq:fourth_order_dyn_II},\,\dummyx_0=\xz,\\
			\dummyx_t \in \Mbb,\text{ and }\dummyu_t \in \Ubb\\
           \quad \text{for all }(w_t,t) \in [-0.01,0.01] \times \timestamp{0}{\horizon-1},\\
            {W} \Let (w_0,\ldots,w_{\horizon-1}),
		\end{cases}
	\end{aligned}
\end{equation}
where \(\Mbb \Let \aset[]{\dummyx \in \Rbb^2 \suchthat \|\dummyx\|_{\infty} \le 5}\) and \(\Ubb \Let \aset[]{\dummyu \suchthat |\dummyu| \le 0.2}\), \(Q \Let I_{4 \times 4}\) is a \(4 \times 4\)-identity matrix, \(R \Let 0.2\).} To find the explicit control law we employed the MPT Toolbox \cite{ref:MPT} with \(w_t=0\), which terminated unsuccessfully around \(5\times 10^4\) regions and was not able to compute the explicit feedback. Keeping the disturbance element \(w_t\) as above and applying the explicit synthesis algorithm reported in \cite{ref:DePena_Explicit_minmax} and \cite{ref:Gao:EMPC}, we observed that the algorithm terminated unsuccessfully as well without being able to compute the explicit feedback due to \textcolor{blue}{a large number of regions} and the corresponding vertex enumeration procedure.

We then deployed our QuIFS algorithm. We fix an approximation error \(\eps \Let 0.05\), i.e., \(\|v_t\|_{\infty} \le 0.05\). Define \(\widetilde{w}_t \Let w_t+Bv_t\) and let \(\widetilde{W} \Let \Wbb \oplus B \Vbb\). The ensuing approximation-ready OCP reads as: 
\textcolor{blue}{\begin{equation}
	\label{eq:approx_ready_RMPC_fourth_order_II}
	\begin{aligned}
		&  \inf_{(\pi_t)_{t=0}^{\horizon-1}} \sup_{\mathsf{W}} && \sum_{t=0}^{\horizon-1} \inprod{\dummyx_t}{Q\dummyx_t} + \inprod{\dummyu_t}{R\dummyu_t} \\
		& \sbjto && \begin{cases}
	\dummyx_{t+1}=A\dummyx_t+B(\dummyu_t+\dummyv_t)+\dummyw_t,\,\dummyx_0=\xz,\\
			\dummyx_t \in \Mbb,\text{ and }\dummyu_t + \dummyv_t \in \Ubb \\
          \quad \text{for all }(\widetilde{w}_t,t) \in \widetilde{W} \times  \timestamp{0}{\horizon-1},\\
            \mathsf{W} \Let (\widetilde{w}_0,\ldots,\widetilde{w}_{\horizon-1}).
		\end{cases}
	\end{aligned}
\end{equation}}
We kept the same computer/server specifications as in Example \eqref{exmp:lmpc_1}, and employed the solver MOSEK along with YALMIP's robust optimization framework to solve the problem \eqref{eq:approx_ready_RMPC_fourth_order_II} using disturbance feedback parameterization of the control policy \cite[Eq. 12a]{ref:Lof:minmax:cdc} at grid points of the underlying state space, with the grid size \(h = 0.01\) (specified below) dictated by the QuIFS algorithm and per point computation time was \(\sim\) 5 sec.
% We performed our numerical computations on MATLAB 2019b using the parallel computation toolbox in an \(36\) core server with Intel(R) Xeon(R) CPU E\(5-2699\) v\(3\), \(4.30\) GHz with \(128\) Gigabyte of RAM. Corresponding to the step size \(h=0.01\) we solved the optimization problem \eqref{eq:approx_ready_RMPC_fourth_order_II} \textcolor{red}{at around \(1\times 10^{7}\) grid points}, where computation-time per point were around \(0.3\) secs.
% this took us around \(16.66\) hours when with the specified server running with \(10\) threads and \(5\) users.
For us the dimension of the state-space \(d=4\). Selecting \(M_0=3\) and using \eqref{num:lagueere_pol}-\eqref{num:high_order_basis}, we get \(\mathsf{L}_2^2 (\dummyx) \Let 6 - 4 \dummyx + \tfrac{\dummyx^2}{2}\) and consequently 
\begin{align}\label{num:sixth_order_basis_nmpc}
      \hspace{-2mm} \Rbb^4 \ni  x \mapsto \psi_6(x) \Let \frac{1}{\pi^2} \left( 6- 4 \|x\|^2+ \frac{1}{2}\|x\|^4\right)\epower{-\|x\|^2}.
    \end{align}
The generating function \eqref{num:sixth_order_basis_nmpc} satisfies the moment condition of order \(M=6\), which means that the constant \(C_{\gamma} = 1/7\). Next, we fix the shape parameter \(\Dd = 2\), and we obtain the value of \(h = \frac{\varepsilon}{3C_\gamma L_0\sqrt{\Dd}} \approx 0.01\), where we have employed a conservative estimate of the Lipschitz constant \(L_0 = 8\) of \(\upopt(\cdot)\). \textcolor{blue}{Define \(\overline{z} \Let x-mh\). We picked \(\rzero=5\), which means that \(11\) terms are used in the quasi-interpolation formula:
\begin{align}\label{num:sixth_quasi_interpolant}
     \mutrunc(x) \Let\hspace{-1mm} \frac{1}{(\pi\Dd)^2}\hspace{-1mm}\sum_{mh \in \finset_x(\rzero)}\hspace{-4mm}\upopt(mh) \biggl( 6 - 4 \frac{\|\overline{z}\|^2}{h^2\Dd}+\frac{1}{2}\frac{\|\overline{z}\|^4}{h^4 \Dd^2}\biggr) \epower{-\frac{\|\overline{z}\|^2}{\Dd h^2}}
 \end{align}
for the approximate feedback synthesis.} Consequently, it is guaranteed that with the approximant \(\mutrunc(\cdot)\) in \eqref{num:sixth_quasi_interpolant} and \((h,\Dd)=(0.01,2)\) the estimate \(\|\upopt(\cdot)-\mutrunc(\cdot)\|_{\mathrm{u}} \le 0.05\) holds.
% Table \eqref{tab:error_margin_LMPC_ex_0} shows a list of parameters \((h,\Dd)\) needed to achieve the presepcified error margin \(\eps\).
% \begin{table}[htbp]
%   \centering
% \caption{\(\eps\) and the pair \(\big(h,\mathcal{D}\bigr)\) associated with example \eqref{eq:RMPC_fourth_order_II}}
%   \begin{tabular}{lccc}
%         \toprule
%           Threshold (\(\eps\))  & \(h\) & \(\mathcal{D}\)                 \\
%         \midrule
%            \( 10 \times 10^{-2} \) & \(0.02\)  & \(2\)                   \\
%           \( 5 \times 10^{-2} \) & \(0.01\)  & \(2\)                   \\
%          %\( 1 \times 10^{-2} \) & \(0.002\)  & \(2\)                 \\
%         \bottomrule
%     \end{tabular}
%   \label{tab:error_margin_LMPC_ex_0}
% \end{table}
We compare our results with the online receding horizon control trajectory. Observe that our results are visibly better than the one reported in \cite[Fig. 6(c)]{ref:summers-multires} in terms of closeness between the online RHC and the approximate trajectory and the error characteristics.
% \begin{table}[htbp]
%   \centering
% \caption{computation-time \textbf{CT} (in secs) and storage requirements (in MB) for the explicit control law}
% \begin{tabular}{lccc}
% \toprule
% Method  & \textbf{CT} (trajectories) & \textbf{CT} \(\bigl(\mutrunc(\cdot)\bigr)\) & Storage 
% \\ \midrule
% QuIFS & 0.007 & 351 & 9        
% \\
% MPT \cite{ref:DePena_Explicit_minmax, ref:MPT} &  Terminated & Terminated  & Terminated
% \\ \bottomrule
%     \end{tabular}
%   \label{tab:metadata_ex_0}
% \end{table}
\textcolor{blue}{The storage requirements, the computation-time to generate the feedback map \(\mutrunc(\cdot)\), and the online computation-time are recorded in Table \eqref{tab:metadata_ex_0} for horizon \(N=17\). Similar statistics with \(N=6\) are given in Table \ref{tab:metadata_new_ex_0}. Figure \eqref{fig:ex_2_fourth_x1_to_x4} depicts the state trajectories and Figure \eqref{fig:ex_2_fourth_u} shows the online receding horizon and the approximate (explicit) control trajectories along with the error between them obtained from QuIFS on the same time scale.} 
% \begin{figure}[h]
% \includegraphics[width=9cm,height=5cm]{Figures/x1x2_error_sum_new.eps}
% \hspace{\fill}
% \includegraphics[width=9cm,height=5cm]{Figures/x3x4_error_sum_new.eps}
% \caption{Closed-loop state trajectories starting from \(x(0) \Let (1,4,1,-1)^{\top}\). QuIFS performs better in comparison to the trajectories reported in \cite[Fig. 6(a) and Fig. 6(b)]{ref:summers-multires}; see the state trajectories, and especially the errors in there. }\label{fig:ex_2_fourth_x1_to_x4}
% \end{figure}
% %%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
\includegraphics[scale=0.4]{Figures/u_error_sum_new.eps}
\caption{The online receding horizon control and the solution obtained from QuIFS for Example \ref{exmp:lmpc_0}. See \cite[Fig. 6(c)]{ref:summers-multires} for a comparison.}\label{fig:ex_2_fourth_u}
\end{figure}
%%%%%%%%
\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
Method  & \textbf{CT} \(\bigl(\mutrunc(\cdot)\bigr)\) & \textbf{CT} (online) & Storage \\ 
\midrule
QuIFS &  187 sec & 5 m.sec & 9 MB        
\\
 MPT \cite{ref:MPT} &  Terminated & NA & Terminated \\ 
 \cite{ref:DePena_Explicit_minmax, ref:Gao:EMPC} & unsuccessfully & & unsuccessfully \\
\bottomrule
    \end{tabular}
    \caption{Computation-time \textbf{CT} and storage requirements with horizon \(\horizon=17\) and \(\eps=0.05\) for Example \ref{exmp:lmpc_0}.}
  \label{tab:metadata_ex_0}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
Method  & \textbf{CT} \(\bigl(\mutrunc(\cdot)\bigr)\) & \textbf{CT} (online) & Storage \\ 
\midrule
QuIFS &  78 sec & 1 m.sec & 0.9 MB \\
\cite{ref:DePena_Explicit_minmax} & 120 sec  & 10 m.sec & 0.5 MB \\ 
 \cite{ref:Gao:EMPC} & 90 sec &  2 m.sec & 0.7 MB  \\
\bottomrule
\end{tabular}
\caption{Computation-time \textbf{CT} and storage requirements with horizon \(\horizon=6\) and \(\eps=0.05\) for Example \ref{exmp:lmpc_0}.}
\label{tab:metadata_new_ex_0}
\end{table}
\end{example}



==> Num_Ex_1.tex <==

%%%%%%%%%%%%%%%%%%
%%% LMPC EX 1 %%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\begin{example}\label{exmp:lmpc_1}
\begin{figure*}[h]
\centering
  \begin{subfigure}[b]{0.5\linewidth}
    \includegraphics[scale=.45]{Figures/without_lip_ext.eps}
  \end{subfigure}
   \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[scale=.45]{Figures/lip_ext.eps}
  \end{subfigure}
\caption{The absolute error between \(\upopt(\cdot)\) and \(\mutrunc(\cdot)\) in Example \ref{exmp:lmpc_1} without the employment of the Lipschitz extension algorithm on the left and with it on the right. Notice that the vertical axis is scaled by the factor of \(10^{-3}\). While in the first case the preassigned error margin \(\eps\) was respected, this may not be typical, and the extension procedure should be carried out in order to conform to the theoretical guarantees.}\label{fig:error_lmpc_ex_1}
\end{figure*}
We start with a two-dimensional example in the linear regime for two specific reasons: (a) to depict the approximation error characteristics, and (b) to show the efficacy of the Lipschitz extension procedure. To this end, for simplicity, we start with a system without any external disturbance, i.e., \(w_t = 0\) (in Example \eqref{exmp:lmpc_0} we consider a noisy dynamical system), but we synthesize (according to the QuIFS algorithm) the approximation-ready policy by translating the nominal MPC problem to a minmax problem. Consider the discrete-time linear time-invariant dynamics \cite{ref:chen2018approximating}:
\begin{equation}\label{eq:exmp_1_dyn}
\st_{t+1}= \begin{pmatrix}
1 & 0.1 \\ 0 & 1
\end{pmatrix} \st_t + \begin{pmatrix}
0.005 \\ 0.1
\end{pmatrix} \ut_t.
\end{equation}
Fix a time horizon \(\horizon \Let 15\) and consider the following finite-horizon discrete-time optimal control problem
    %  \begin{align}\label{eq:exmp_1_linear-original problem}
    %     \begin{aligned}
    %     &\minimize_{(\dummyu_t)_{t=0}^{\horizon-1}}  && \sum_{t=0}^{\horizon-1}\inprod{\dummyx_t}{Q\dummyx_t}+\inprod{\dummyu_t}{R\dummyu_t}\\
    %         &\sbjto && \begin{cases}
    %       \text{dynamics} \,\,\eqref{eq:exmp_1_dyn},\,|\st^1_{t}|\le 6, \\|\st^{2}_{t}|\le 1 \hspace{1mm}\text{for all }t \in \timestamp{0}{\horizon-1},\\
    %         |\ut_t| \le 2 \hspace{3.5mm}\text{for all }t \in \timestamp{0}{\horizon-1},
    %         \end{cases}
    %     \end{aligned}
    % \end{align}
\textcolor{blue}{\begin{align}\label{eq:exmp_1_linear-original problem}
   \hspace{-3mm} \begin{aligned}
        &\inf_{(\dummyu_t)_{t=0}^{\horizon-1}}  && \hspace{-3mm}\sum_{t=0}^{\horizon-1}\inprod{\dummyx_t}{Q\dummyx_t}+\inprod{\dummyu_t}{R\dummyu_t}\\
            &\sbjto && \hspace{-3mm}\begin{cases}
          \text{the dynamics }\eqref{eq:exmp_1_dyn},\,\dummyx_0=\xz,\\
          \dummyx_t \in \Mbb,\text{ and }\dummyu_t \in \Ubb \,\,\text{for all }t \in \timestamp{0}{\horizon-1},
            \end{cases}
        \end{aligned}
    \end{align}
where \(\Mbb \Let \aset[]{(\dummyx_1,\dummyx_2) \in \Rbb^2 \suchthat |\dummyx_1|\le 6,\,|\dummyx_2|\le 1}\), \(\Ubb \Let \aset[]{\dummyu \in \Rbb \suchthat |\dummyu|\le 2}\).} The state weighting matrix \(Q\) is the \(2\times 2\) identity matrix and the control weighting matrix is \(R \Let 1\). The policy \(\upopt(\cdot)\) at points was obtained by gridding the state-space \([-6,6] \times [-1,1] \) with a cardinal grid of step size \(h=0.0035\). We performed our numerical computations on MATLAB 2019b using the parallel computation toolbox in an \(36\) core server with Intel(R) Xeon(R) CPU E\(5-2699\) v\(3\), \(4.30\) GHz with \(128\) Gigabyte of RAM, and we employed the solver MOSEK \cite{ref:mosek} along with the robust optimization module \cite{ref:lofberg2012automatic} in YALMIP \cite{ref:YALMIP_lofberg2004} to solve the problem \eqref{eq:exmp_1_linear-original problem} where per point computation-time was \(\sim\) \(1.5\) sec. 
%which took around \(1.5\) hours.
It turns out that the Lipschitz constant of \(\upopt(\cdot)\) is bounded above by \(L_{0} \approx 2 \). For the quasi-interpolation scheme, we picked the Laguerre polynomial-based basis function given by:
\begin{align}\label{num:high_order_basis}
    \psi_{2M_0}(x) \Let \pi^{-d/2}\mathsf{L}_{M_0-1}^{d/2}\big(\|x\|^2\bigr)\epower{-\|x\|^2},
\end{align}
where the Laguerre polynomials are given by
\begin{align}\label{num:lagueere_pol}
    \mathsf{L}^{j}_{k}(x) \Let \frac{x^{-j}}{k!}\epower{x} \left(\frac{\dd}{\dd x}\right)^k(x^{k+j}\epower{x}), \,j>-1.
\end{align}
In \cite{ref:maz_mfld} it is shown that a \(d\)-dimensional approximant of the form \eqref{eq:approx_policy} with the basis \eqref{num:high_order_basis} leads to uniform approximation of order \(M \Let 2M_0\), i.e., \(\mathcal{O}(h^{2M_0})\), where \(M_0=1,2,\ldots\), and \(M\) is the order of the moment condition; (see \eqref{eq:moment_condition}). The Laguerre-Gaussian basis function, i.e., \eqref{num:high_order_basis} with \(d=2\) and \(M_0 = 3\) is given by
\begin{align}\label{num:sixth_order_basis_ex_1}
   \hspace{-1mm} \Rbb^2 \ni   x \mapsto \psi(x) \Let \frac{1}{\pi} \left( 3- 3 \|x\|^2+ \frac{1}{2}\|x\|^4\right)\epower{-\|x\|^2}
    \end{align}
that satisfies a moment condition of order \(M=6\), and thus \(C_{\gamma}=1/6\). For illustration, let us fix an error tolerance \(\eps= 0.005\). Fix the shape parameter \(\Dd = 2\) and simple algebra leads to the parameter \(h = \frac{\eps}{3C_{\gamma}L_{0}\sqrt{\Dd}} = 0.004\). Define \(\overline{z} \Let x-mh\). We choose \(\rzero=3\), i.e., 7 terms are used at each \(x\) in the following quasi-interpolant:
\begin{align}\label{quasi_lmpc_ex_1}
     \mutrunc(x) \Let \frac{1}{\pi\Dd}\sum_{mh \in \finset_x(\rzero)}\hspace{-3mm}\upopt(mh) \,\biggl( 3 - 3 \frac{\|\overline{z}\|^2}{h^2\Dd}+\frac{1}{2}\frac{\|\overline{z}\|^4}{h^4 \Dd^2}\biggr) \epower{-\frac{\|\overline{z}\|^2}{\Dd h^2}}.
\end{align}
It is guaranteed that for the given \(\eps= 0.005\), our one-shot synthesis produces the pair \(\bigl(h,\Dd\bigr)=\bigl(0.004,2\bigr)\) such that \(\|\upopt(\cdot)- \mutrunc(\cdot)\|_{\mathrm{u}}\le 0.005\). Figure \eqref{fig:error_lmpc_ex_1} numerically verifies this fact. Table \eqref{tab:error_margin_LMPC_ex_1} shows a list of user-defined tolerance values and the corresponding \(h\) and \(\Dd\) needed to achieve it. \textcolor{blue}{Although the error tolerance \(\eps\) between \(\upopt(\cdot)\) and \(\mutrunc(\cdot)\) was respected (see left-hand subfigure in Figure \ref{fig:error_lmpc_ex_1}) even before the Lipschitz extension, we employed the Lipschitz extension algorithm described in \S\ref{sec:extension_algo} to illustrate its positive effects. To this end, we set \(\rzero = 50\) and pre-calculated all the values of \(\upopt(\cdot)\) both inside \(\widehat{X}_N\) (an \(h\)-net of \(X_N\)) and outside of \(\widehat{X}_N\) via \eqref{eq:extented_policy} and subsequently we employed the approximation scheme \eqref{quasi_lmpc_ex_1} to generate \(\mutrunc(\cdot)\) and restricted it to \(\widehat{X}_N\) eventually. Compared to the left-hand subfigure of Figure \eqref{fig:error_lmpc_ex_1}, is it clear that the error reduced significantly after the extension algorithm was employed. The corresponding storage and computation-time requirements are recorded in Table \eqref{tab:metadata_ex_1}.} 
%%% Feedback plots %%%
% \begin{figure}[!hb]
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{Figures/draft_lmpc_ex_1_uopt.eps}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{Figures/draft_lmpc_ex_1_uhat.eps}
%   \end{subfigure}
%  \caption{The optimal feedback \(\upopt(\cdot)\) and the approximated feedback \(\mutrunc(\cdot)\) for Example \eqref{exmp:lmpc_1} with \(\eps=0.005\), and \(\bigl(h,\Dd \bigr)=(0.0035,2)\). }\label{fig:uopt_uapp_lmpc_ex_1}
% \end{figure}
%%% Error plots %%%
% \begin{figure}[!hb]
%   \centering
%   \begin{subfigure}[b]{0.48\linewidth}
%     \includegraphics[width=\linewidth]{Figures/with_LipE_draft_lmpc_ex_1_abs_error.eps}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.48\linewidth}
%     \includegraphics[width=\linewidth]{Figures/without_LipE_draft_lmpc_ex_1_abs_error.eps}
%   \end{subfigure}
% \caption{The absolute error between \(\upopt(\cdot)\) and \(\mutrunc(\cdot)\) with the employment of the Lipschitz extension algorithm on the left and without it on the right. Notice that the vertical axis is scaled by the factor of \(10^{-3}\).}\label{fig:error_lmpc_ex_1}
% \end{figure}
%%%%%%%%%%%%%%%
 \begin{table}[b]
  \centering
  \begin{tabular}{lccc}
        \toprule
          Threshold (\(\eps\))  & \(h\) & \(\mathcal{D}\)                 \\
        \midrule
           \( 50 \times 10^{-3} \) & \(0.04\)  & \(2\)                   \\
          \( 5 \times 10^{-3} \) & \(0.004\)  & \(2\)                   \\
         % \( 1 \times 10^{-3} \) & \(0.0008\)  & \(2\)                 \\
        \bottomrule
    \end{tabular}
    \caption{The error-margin \(\eps\) and the pair \(\big(h,\mathcal{D}\bigr)\) associated with example \eqref{exmp:lmpc_1}.}
  \label{tab:error_margin_LMPC_ex_1}
\end{table}
%%%%%%%%%%%%%
\begin{table}[b]
  \centering
\begin{tabular}{lccc}
\toprule
Method  & \textbf{CT} \(\bigl(\mutrunc(\cdot)\bigr)\) & \textbf{CT} (online) & Storage 
\\ \midrule
QuIFS & 23 sec  & 0.5 m.sec & 25 KB
\\
MPT \cite{ref:MPT} &  19 sec & 0.8 m.sec & 17 KB
\\ \bottomrule
    \end{tabular}
    \caption{Computation-time \textbf{CT} and storage requirements with \(\eps=0.05\) for Example \ref{exmp:lmpc_1}.}
  \label{tab:metadata_ex_1}
\end{table}
\end{example}
\begin{figure*}[htbp]
  \begin{subfigure}[b]{0.5\linewidth}
    \includegraphics[scale=0.45]{Figures/x1x2_error_sum_new.eps}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[scale=0.45]{Figures/x3x4_error_sum_new.eps}
  \end{subfigure}
\caption{Closed-loop state trajectories starting from \(x(0) \Let (1,4,1,-1)^{\top}\) for Example \ref{exmp:lmpc_0}. QuIFS performs better in terms of closeness to the online RHC trajectories in comparison to the trajectories reported in \cite[Fig. 6(a) and Fig. 6(b)]{ref:summers-multires}; see the state trajectories, and especially the errors in there.}\label{fig:ex_2_fourth_x1_to_x4}
\end{figure*}

==> Num_Ex_2.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%% LMPC EX 2 %%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\noindent We provide a second example in the linear MPC regime.
\begin{example}\label{exmp:lmpc_2}
 Consider the following discrete time non-autonomous dynamics \cite{ref:BemMorDuaPis-02}:
    \begin{equation}\label{eq:exmp_2_dyn}
    \st_{t+1}= \begin{pmatrix}
            1 & 1 \\ 0 & 1
        \end{pmatrix}  \st_{t}+ \begin{pmatrix}
                1 \\ 0.5
            \end{pmatrix} \ut_t.
    \end{equation}
    Fix the horizon \(\horizon \Let 10\) and consider the following finite horizon discrete-time optimal control problem
     \begin{align}\label{eq:exmp_2_linear-original problem}
        \begin{aligned}
            &\inf_{(\ut_t)_{t=0}^{\horizon-1}}  && \sum_{t=0}^{\horizon-1}\inprod{\st_t}{Q\st_t}+\inprod{\ut_t}{R \ut_t}\\
            &\sbjto && \begin{cases}
          \text{dynamics} \,\,\eqref{eq:exmp_2_dyn},\\
            |\st_t| \le 5 \quad\text{for \,} t=0,\ldots,\horizon-1,\\
            |\ut_t| \le 1 \quad\text{for \,} t=0,\ldots,\horizon-1,
            \end{cases}
        \end{aligned}
    \end{align}
    where the weighting matrices are \[Q \Let \begin{pmatrix}0.1&0\\0&2 \end{pmatrix}, \,\,R \Let 1.\] 
We used YALMIP with the QP solver \(\mathsf{quadprog}\) to solve the problem \eqref{eq:exmp_2_linear-original problem} and the optimal solution was obtained by gridding the state-space \([-5,5] \times [-5,5] \) with step size \(h=0.0017\); see the left sub-figure in Figure \eqref{fig:uopt_uapp_lmpc_ex_2}. Since we did not have a sharp error variations near boundary, we skipped the extension procedure for this example. For the quasi-interpolation \eqref{eq:approx_policy} we picked the basis function in
\eqref{num:2nd_order_basis}. We choose \(R_0=5\); i.e., only 11 terms are used in the approximation formula \eqref{num:2nd_quasi_interpolant} around each \(x\). The Lipschitz constant of \(u\as_0(\cdot)\) is, as before, roughly \(L_{0} \approx 1 \). Let us fix an error tolerance \(\eps= 0.0025\); fix the shape parameter \(\Dd = 2\), simple algebra leads to the parameter \(h =  \frac{\eps}{3C_{\gamma}L_{0}\sqrt{\Dd}} = 0.0017 \). Figure \eqref{fig:error_lmpc_ex_2} numerically verifies the uniform error margin \(\unifnorm{u_0\as-\widehat{u}_0} \le 0.0025\). Table \eqref{tab:error_margin_LMPC_ex_2} shows a list of user-defined tolerance values and the corresponding \(h\) and \(\Dd\) needed to achieve it.
 \begin{table}[htbp]
  \centering
\caption{The error-margin \(\eps\) and the pair \(\big(h,\mathcal{D}\bigr)\) associated with example \eqref{exmp:lmpc_2}}
  \begin{tabular}{lccc}
        \toprule
          Threshold (\(\eps\))  & \(h\) & \(\mathcal{D}\)                 \\
        \midrule
           \( 10 \times 10^{-3} \) & \(0.0070\)  & \(2\)                   \\
          \( 2.5 \times 10^{-3} \) & \(0.0017\)  & \(2\)                   \\
         \( 1 \times 10^{-3} \) & \(0.0007\)  & \(2\)                 \\
        \bottomrule
    \end{tabular}
  \label{tab:error_margin_LMPC_ex_2}
\end{table}
 Corresponding to the error-margin \(\eps=0.0025\), the actual and the approximate feedback functions are depicted in Figure \eqref{fig:uopt_uapp_lmpc_ex_2} and the error surface is shown in Figure \eqref{fig:error_lmpc_ex_2}. It can be clearly observed that the error tolerance \(\eps=0.0025\) is respected with our particular choice of the pair \(\bigl(h,\Dd\bigr)\).
%%% Feedback plots %%%

\begin{figure}[!ht]
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{Figures/LMPC_Ex_2_u_opt.eps}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{Figures/LMPC_Ex_2_u_app.eps}
  \end{subfigure}
 \caption{The optimal feedback \(u^*_0\) computed at points by means of YALMIP and the approximated feedback \(\widehat{u}_0\) corresponding to Example \eqref{exmp:lmpc_2} with \(\eps=0.0025\), and \(\bigl(h,\Dd \bigr)=(0.0017,2)\) obtained from Table \eqref{tab:error_margin_LMPC_ex_2}.}\label{fig:uopt_uapp_lmpc_ex_2}
\end{figure}

% \begin{figure}[ht]
% \includegraphics[width=0.48\textwidth]{Figures/LMPC_Ex_2_u_opt.eps}
% \hspace{\fill}
% \includegraphics[width=0.48\textwidth]{Figures/LMPC_Ex_2_u_app.eps}
% \caption{The optimal feedback \(u^*_0\) computed at points by means of YALMIP and the approximated \(\widehat{u}_0\) feedback functions corresponding to Example \eqref{eq:exmp_2_linear-original problem} with \(\eps=0.0025\), and \(\bigl(h,\Dd \bigr)=(0.002651,4)\).}\label{fig:uopt_uapp_lmpc_ex_2}
% \end{figure}

%%% Error plots %%%
\begin{figure}[ht]
\includegraphics[width=9cm,height=6cm]{Figures/LMPC_Ex_2_Abs_Error.eps}
\caption{The absolute error between the actual and the approximated feedback functions corresponding to Example \eqref{exmp:lmpc_2} without the Lipschitz extension procedure. Notice that the vertical axis is scaled by the factor of \(10^{-3}\) and the tolerance \(\eps=0.0025\) is respected.}\label{fig:error_lmpc_ex_2}
\end{figure}

%%% e,h,D, and the error table %%%

% \begin{table}[h!]
%   \centering
%   \begin{tabular}{ | m{2cm} | m{2cm} | c | }
%     \hline
%   \(\bigl(h,\Dd\bigr)\) & \(\eps\) & Error \\ \hline
%     \( \bigl( 0.25,2 \bigr) \) & 0.1 &
%      \begin{minipage}{.5\textwidth}
%       \includegraphics[width=\linewidth, height=50mm]{ex_2_err_0.eps}
%     \end{minipage}
%     \\ \hline 
%     \( \bigl(0.1,2.5  \bigr) \) & 0.01 & 
%     \begin{minipage}{.5\textwidth}
%       \includegraphics[width=\linewidth, height=50mm]{ex_2_err_1.eps}
%     \end{minipage}
%     \\ 
%     \hline
%     \( \bigl(0.05,5 \bigr)\) & 0.005  & 
%      \begin{minipage}{.5\textwidth}
%       \includegraphics[width=\linewidth, height=50mm]{ex_2_err_2.eps}
%     \end{minipage}
%     \\
%     \hline 
%     % something & something & 
%     %  \begin{minipage}{.5\textwidth}
%     %   \includegraphics[width=\linewidth, height=50mm]{Figures_Num_Ex_2/ex_2_err_4.eps}
%     % \end{minipage}
%     % \\ 
%     % \hline 
%   \end{tabular}
%   \caption{The error plots corresponding to the pair \(\bigl(h,\Dd\bigr)\) and the fixed tolerance \(\eps\)}\label{tbl:num_ex_2_errors}
% \end{table}
\end{example}




==> Num_Ex_3.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%% NMPC EX 1 %%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%

\begin{example}\label{exmp:nmpc_1}
Consider the dynamical system \cite{Raimondo2012}:
\begin{align} \label{eq:nonlinear_example}
   \dot{\st}_1(t)&=\st_2(t)+ \bigl(0.5 +0.5 \st_1(t) \bigr)\ut(t) \nn \\\dot{\st}_2(t) &= \st_1(t)+ \bigl(0.5 -2\st_2(t) \bigr)\ut(t).
\end{align}
We discretize the system dynamics \eqref{eq:nonlinear_example} using a Runge-Kutta (RK4) discretization scheme with sampling time \(T_s \Let 0.1\). For a fixed time horizon \(\horizon \Let 15\), consider the finite horizon discrete-time optimal control problem 
 % \begin{align}\label{eq:exmp_2_nonlinear-original problem}
 %        \begin{aligned}
 %            &\minimize_{(\ut_t)_{t=0}^{\horizon-1}}  && \hspace{-2mm}\inprod{\st_N}{P\st_N}+\sum_{t=0}^{\horizon-1}\inprod{\st_t}{Q\st_t}+\inprod{\ut_t}{R\ut_t}\\
 %            &\sbjto && \hspace{-2mm}\begin{cases}
 %          \text{discretized dynamics} \,\,\eqref{eq:nonlinear_example},\,x_N \in \Mbb_F,\\
 %            |\st_t| \le 1,\, |\ut_t| \le 2 \text{ for all }t \in \timestamp{0}{\horizon-1},
 %            \end{cases}
 %        \end{aligned}
 %    \end{align}
 \textcolor{blue}{\begin{align}\label{eq:exmp_2_nonlinear-original problem}
        \begin{aligned}
            &\inf_{(\dummyu_t)_{t=0}^{\horizon-1}}  && \hspace{-2mm}\inprod{\dummyx_N}{P\dummyx_N}+\sum_{t=0}^{\horizon-1}\inprod{\dummyx_t}{Q\dummyx_t}+\inprod{\dummyu_t}{R\dummyu_t}\\
            &\sbjto && \hspace{-2mm}\begin{cases}
          \text{discretized dynamics }\eqref{eq:nonlinear_example},\,\dummyx_0= \xz,\\
            \dummyx_t \in \Mbb,\,\dummyx_{\horizon} \in \Mbb_F \text{ and }\dummyu \in \Ubb\text{ for all }t \in \timestamp{0}{\horizon-1},
            \end{cases}
        \end{aligned}
    \end{align}
where \(\Mbb \Let \aset[]{\dummyx \in \Rbb^2 \suchthat \|\dummyx\|_{\infty} \le 1}\), \(\Ubb \Let \aset[]{\dummyu \in \Rbb \suchthat |\dummyu| \le 1}\),} \(Q \Let 0.01 I_{2\times 2}\), \(R\Let 0.01\), and \(P \Let \begin{psmallmatrix}19.6415&13.1099 \\13.1099&19.6414
\end{psmallmatrix}\), which is found by solving the Lyapunov equations \cite{Raimondo2012}. The terminal region is \(\Mbb_{F} \Let \aset[\big]{\st \in \Rbb^2 \mid \inprod{\st}{P\st} \le 1}.\) The solution to \eqref{eq:exmp_2_nonlinear-original problem} is obtained by gridding the state-space \([-1,1] \times [-1,1] \) with step size \(h=0.0035\) (dictated by the QuIFS algorithm). We employed the NLP solver \(\mathsf{IPOPT}\) in YALMIP with the same computer specifications as in Example \eqref{exmp:lmpc_1} to solve the optimization problem \eqref{eq:exmp_2_nonlinear-original problem}, where per point computation-time was \(\sim\) \(3\) sec. The Lipschitz constant of \(\upopt(\cdot)\) is roughly \(L_{0} \approx 2\) as estimated by numerical techniques. For the quasi-interpolation scheme we choose the Laguerre generating function by fixing \(M_0=5\) and \(d=2\) in \eqref{num:high_order_basis}
% \begin{figure*}[h]
% \centering
%   \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[scale=0.3]{Figures/x1x2_opt_app_summ.eps}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.3\linewidth}
%     \includegraphics[scale=0.3]{Figures/u_new_summ_II.eps}
%   \end{subfigure}
% \caption{State trajectories generated by QuIFS, the algorithm reported in \cite{Raimondo2012}, and the online receding horizon state trajectories for \(x_0 \Let \begin{pmatrix}-0.7&-0.85 \end{pmatrix}^{\top}\) (left) and the control trajectories, for a simulation length \(120\).}\label{fig:raimondo_state_control}
% \end{figure*}
\begin{align}\label{num:tenth_order_basis}
      & \Rbb^2 \ni x \mapsto \psi_{10}(x) \Let \frac{1}{\pi} \big{(} 5- 10\|x\|^2 +5\|x\|^4-\frac{5}{6}\|x\|^6  \nn \\& +\frac{1}{24}\|x\|^8\big{)}\epower{-\|x\|^2}.
\end{align}
which satisfies moment condition of order \(M=10\), and consequently \(C_{\gamma} = 1/11\). For illustration, let us fix a error tolerance \(\eps= 0.005\), and fix the shape parameter \(\Dd = 2\). Simple algebra leads to the parameter \(h = \frac{\eps}{3C_{\gamma}L_{0}\sqrt{\Dd}} = 0.0063\). Observe that the value of \(h\) is conservative in nature, and it may be possible to achieve the error tolerance with higher values of \(h\). We choose \(R_0=7\), and employ the quasi-interpolant \eqref{quasi_lmpc_ex_1} with \(\psi_{10}(\cdot)\) in place of \(\psi(\cdot)\) to generate the approximate policy \(\mutrunc(\cdot)\) and it is guaranteed that the pair \(\bigl(h,\Dd\bigr)=\bigl(0.0063,2\bigr)\) leads to \(\|\upopt(\cdot)-\mutrunc(\cdot)\|_{\mathrm{u}} \le 0.005\). Figure \eqref{fig:error_nmpc_ex_2} numerically verifies this fact. 
% Table \eqref{tab:error_margin_NMPC_ex_2} shows a list of user-defined tolerance values and the corresponding \(h\) and \(\Dd\) needed to achieve them. 
%  \begin{table}[htbp]
%   \centering
% \caption{The error-margin \(\eps\) and the pair \(\big(h,\mathcal{D}\bigr)\) associated with example \eqref{exmp:nmpc_1}}
%   \begin{tabular}{lccc}
%         \toprule
%           Threshold (\(\eps\))  & \(h\) & \(\mathcal{D}\)                 \\
%         \midrule
%            \( 50 \times 10^{-3} \) & \(0.0643\)  & \(2\)                   \\
%           \( 10 \times 10^{-3} \) & \(0.0129\)  & \(2\)                   \\
%          % \( 5 \times 10^{-3} \) & \(0.0063\)  & \(3\)                 \\
%         \bottomrule
%     \end{tabular}
%   \label{tab:error_margin_NMPC_ex_2}
% \end{table}
Corresponding to the error margin \(\eps=0.005\), the error surface is shown in Figure \eqref{fig:error_nmpc_ex_2}. Table \eqref{tab:metadata_nl_ex_1} records computation-time and storage requirements corresponding to an error margin \(\eps = 0.05\).
%%% Feedback plots %%%
% \begin{figure}[!ht]
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{Figures/NMPC_Ex_1_uopt.eps}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{Figures/NMPC_Ex_1_uapp.eps}
%   \end{subfigure}
%  \caption{The optimal feedback \(\upopt(\cdot)\) and the approximated feedback \(\mutrunc(\cdot)\) for Example \eqref{exmp:nmpc_1} with \(\eps=0.005\), and \(\bigl(h,\Dd \bigr)=(0.0063,2)\).}\label{fig:uopt_uapp_nmpc_ex_2}
% \end{figure}

% \begin{figure}[ht]
% \includegraphics[width=0.48\textwidth]{Figures/NMPC_Ex_1_uopt.eps}
% \hspace{\fill}
% \includegraphics[width=0.48\textwidth]{Figures/NMPC_Ex_1_uapp.eps}
% \caption{The optimal feedback \(u^*_0\) computed at points by means of YALMIP and the approximated \(\widehat{u}_0\) feedback functions corresponding to Example \eqref{eq:exmp_1_linear-original problem} with \(\eps=0.005\), and \(\bigl(h,\Dd \bigr)=(0.005336,4)\).}\label{fig:uopt_uapp_nmpc_ex_2}
% \end{figure}
%%% Error plots %%%%
\begin{figure}[t]
\includegraphics[scale=0.4]{Figures/nmpc_abs_error_005.eps}
\caption{The absolute error between \(\upopt(\cdot)\) and \(\mutrunc(\cdot)\) for Example \eqref{exmp:nmpc_1}.}\label{fig:error_nmpc_ex_2}
\end{figure}
%%%% colin raimondo state con traj %%%%
\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{Figures/x1x2_opt_app_summ.eps}
\caption{State trajectories for Example \eqref{exmp:nmpc_1} generated by QuIFS, the algorithm reported in \cite{Raimondo2012}, and the online receding horizon state trajectories for \(x_0 \Let \begin{pmatrix}-0.7&-0.85 \end{pmatrix}^{\top}\) for a simulation length \(120\).}\label{fig:raimondo_state}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{Figures/u_new_summ_II.eps}
\caption{Control trajectories for Example \eqref{exmp:nmpc_1} generated by QuIFS, the algorithm reported in \cite{Raimondo2012}, and the online receding horizon control trajectory for a simulation length \(120\). }\label{fig:raimondo_control}
\end{figure}
Moreover, it can be seen (see the enlarged snippets within the figures) that in terms of closeness to the online RHC trajectories QuIFS does a better job compared to the hierarchical grid-based technique reported in \cite{Raimondo2012}. Indeed, there is visibly less oscillatory behaviour under QuIFS compared to \cite{Raimondo2012}. 
\begin{table}[!h]
  \centering
\begin{tabular}{lccc}
\toprule
Method  & \textbf{CT} \(\bigl(\mutrunc(\cdot)\bigr)\) & \textbf{CT} (online) & Storage 
\\ \midrule
QuIFS & 77 sec  & 0.4 m.sec & 34 KB \\
\cite{Raimondo2012} & 61 sec & 0.7 m.sec & 30 KB
\\ \bottomrule
    \end{tabular}
    \caption{Computation-time \textbf{CT} and storage requirement with \(\eps=0.05\) for Example \eqref{exmp:nmpc_1}.}
  \label{tab:metadata_nl_ex_1}
\end{table}
\end{example}

% \section{Acknowledgement}
% \textcolor{blue}{We sincerely thank one of the anonymous reviewers for providing relevant references and pointing out several typos and a few technical inconsistencies in the manuscript.}




==> Num_Ex_4.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%% NMPC EX 2 %%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Example 2}
Consider the one dimensional bilinear system \cite{ref:grune2017nonlinear}
\begin{align} \label{eq:nonlinear_2_example}
   x^{+}=x+u+xu 
\end{align}
 We discretize the system dynamics \eqref{eq:nonlinear_2_example} using a Runge-Kutta (RK4) scheme with sampling time \(T_s \Let 0.1\). Fix \(N\Let 10\), and consider the finite horizon discrete-time optimal control problem 
 \begin{align}\tag{Ex-2-NMPC(\(\bar{x})\)}
        \label{eq:exmp_2_nonlinear-original problem}
        \begin{aligned}
            &\minimize_{(u_t)_{t=0}^{N-1}}  && \sum_{t=0}^{N-1}x_t^2+u_t^2+u_t^4\\
            &\hspace{2mm}\sbjto && \begin{cases}
          \text{discretized dynamics} \,\,\eqref{eq:nonlinear_2_example},\\
            x_t \in \Mbb \Let \Rbb\\
            u_t \in \Ubb \Let \Rbb.
            \end{cases}
        \end{aligned}
    \end{align}
  For numerical computation, we choose the one-dimensional version of the basis function in \eqref{num:sixth_order_basis}, with \(\Dd =\Dd(h) \Let 6 |\log h|/\pi^2\), and \(h=0.5\). The actual NMPC optimal feedback and the approximate feedback are shown in Fig.\eqref{fig:16_5_Actual_Approx_NMPC}, and the errors are shown in Fig.\eqref{fig:16_5_Actual_Approx_NMPC_Error}.
\begin{figure}[ht]
\includegraphics[width=0.48\textwidth]{Ex5_16_u_opt_v2.eps}
\hspace{\fill}
\includegraphics[width=0.48\textwidth]{Ex5_16_u_app_v2.eps}
\caption{The actual and the approximated feedback functions}\label{fig:16_5_Actual_Approx_NMPC}
\end{figure}
\begin{figure}[ht]
\includegraphics[width=9cm,height=6cm]{Ex5_16_error_v2.eps}
\caption{The error between the actual and the approximated feedback function}\label{fig:16_5_Actual_Approx_NMPC_Error}
\end{figure}


==> Num_Ex_5.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%% NMPC EX 3 %%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{example}\label{exmp:nmpc_3}
Consider the continuous-time second-order nonlinear controlled dynamical system \cite{ref:canale:sm:approx}: 
\begin{align}\label{eq:nonlinear_3_example}
    \dot{x}_1(t)& = x_2(t) \nn \\ \dot{x}_2(t) & = u(t) - 0.6 x_2(t) -x_1(t)^3 - x_1(t).
\end{align}
\begin{figure*}[h]
  \begin{subfigure}[b]{0.32\linewidth}
    \includegraphics[width=6cm,height=5cm]{Figures/can_u_opt.eps}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\linewidth}
    \includegraphics[width=6cm,height=5cm]{Figures/can_u_app.eps}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=6cm,height=5cm]{Figures/can_new_error.eps}
  \end{subfigure}
\caption{The feedback \(\upopt(\cdot)\), the explicit feedback \(\mutrunc(\cdot)\), and the absolute error between \(\upopt(\cdot)\) and \(\mutrunc(\cdot)\) for Example \eqref{exmp:nmpc_3} with \(\eps=0.05\), and \(\bigl(h,\Dd \bigr)=(0.01,2)\).}\label{fig:can_Actual_Approx_NMPC}
\end{figure*}
The system dynamics \eqref{eq:nonlinear_3_example} is discretized using a forward-Euler scheme with sampling time \(T_s \Let 0.05\). Fix \(\horizon \Let 100\), and consider the finite horizon discrete-time optimal control problem 
% \begin{align}
%         \label{eq:exmp_3_nonlinear-original problem}
%         \begin{aligned}
%             &\min_{(\dummyu_t)_{t=0}^{\horizon-1}}  && \sum_{t=0}^{\horizon-1} \inprod{x_t}{Qx_t}+\inprod{u_t}{Ru_t}\\
%             &\hspace{2mm}\sbjto && \begin{cases}
%           \text{discretized dynamics} \,\,\eqref{eq:nonlinear_3_example},\\
%             |x_t| \le 5,\,|u_t| \le 5 \text{ for all }t \in \timestamp{0}{\horizon-1},
%             %\text{for all }(w_t,t) \in  [-0.01,0.01] \times \timestamp{0}{\horizon-1},
%             \end{cases}
%         \end{aligned}
%     \end{align}
\textcolor{blue}{\begin{align}
        \label{eq:exmp_3_nonlinear-original problem}
        \begin{aligned}
            &\inf_{(\dummyu_t)_{t=0}^{\horizon-1}}  && \hspace{-2mm}\sum_{t=0}^{\horizon-1} \inprod{\dummyx_t}{Q\dummyx_t}+\inprod{\dummyu_t}{R\dummyu_t}\\
            &\sbjto && \hspace{-2mm} \begin{cases}
          \text{discretized dynamics }\eqref{eq:nonlinear_3_example}, \,\dummyx_0 = \xz, \\
          \dummyx_t \in \Mbb, \text{ and }\dummyu_t \in \Ubb
            \text{ for all }t \in \timestamp{0}{\horizon-1},
            %\text{for all }(w_t,t) \in  [-0.01,0.01] \times \timestamp{0}{\horizon-1},
            \end{cases}
        \end{aligned}
    \end{align}
where \(\Mbb \Let \aset[]{\dummyx \in \Rbb^2 \suchthat \|\dummyx\|_{\infty} \le 5}\), \(\Ubb \Let \aset[]{\dummyu \in \Rbb \suchthat |\dummyu| \le 5}\), \(Q \Let \mathbb{I}_{2 \times 2}\), and \(R \Let 0.5\).} Let us fix \(\eps = 0.05 \). For the synthesis of the approximation-ready policy, as per our formulation, we consider the dynamics: 
\begin{align}\label{eq:nonlinear_3_example_noisy}
    \dot{x}_1(t) &= x_2(t), \nn \\
        \dot{x}_2(t) &= u(t) + v(t) -0.6x_2(t)-x_1(t)^3-x_1(t).
\end{align}
Then the approximation-ready robust optimal control problem is 
\textcolor{blue}{\begin{equation}
	\label{eq:approx_ready_RMPC_num_ex_0}
	\begin{aligned}
		&  \inf_{(\dummyu_t)_{t=0}^{\horizon-1}} \sup_{\mathsf{W}} && \sum_{t=0}^{\horizon-1} \inprod{\dummyx_t}{Q\dummyx_t} + \inprod{\dummyu_t}{R\dummyu_t} \\
		& \sbjto && \begin{cases}
			 \text{discretized dynamics }\eqref{eq:nonlinear_3_example_noisy},\,\dummyx_0= \xz,\\
			\dummyx_t \in \Mbb, \text{ and }\dummyu_t + \dummyv_t \in \Ubb \\
           \quad\text{for all } (\dummyv_t,t)\in [-0.05,0.05] \times \timestamp{0}{\horizon-1},\\
            \mathsf{W} \Let (\dummyv_0,\ldots,\dummyv_{\horizon-1}).
		\end{cases}
	\end{aligned}
\end{equation}}
The solution to the problem \eqref{eq:approx_ready_RMPC_num_ex_0} was obtained by gridding the state-space \([-5,5] \times [-5,5] \) with step size \(h=0.01\) and solving the ensuing NLP \eqref{eq:approx_ready_RMPC_num_ex_0} in YALMIP using the NLP solver \(\mathsf{IPOPT}\) \cite{ref:IPOPT_Biegler} deriving a robust counterpart. The problem \eqref{eq:approx_ready_RMPC_num_ex_0} can be alternatively solved using the algorithm reported in \cite{ref:JK:MM:FA:2021} as well. We performed our numerical computation keeping the computer server identical to the one in Example \eqref{exmp:lmpc_1}, and computation-time per point was \(\sim\) \(2.3\) sec. Next we choose the Laguerre-Gaussian basis function with \(d=2\), and \(M_0=3\):
\begin{align}\label{num:sixth_order_basis}
      \Rbb^2 \ni  x \mapsto \overline{\psi}_6(x) \Let \frac{1}{\pi} \left( 3- 3 \|x\|^2+ \frac{1}{2}\|x\|^4\right)\epower{-\|x\|^2}.
    \end{align}
The generating function \(\overline{\psi}_6(\cdot)\) satisfies a moment condition of order \(M=6\), which means that the constant \(C_{\gamma} = 1/7\). Next, we fix the shape parameter \(\Dd = 2\), we obtain the value of \(h = \frac{\varepsilon}{3C_\gamma L_0\sqrt{\Dd}} \approx 0.01\), where \(L_0 = 4\) is a rough estimate of Lipschitz constant of \(\upopt(\cdot)\), estimated numerically. Choosing \(\rzero=3\), we employ the quasi-interpolant \eqref{quasi_lmpc_ex_1} with \(\overline{\psi}_{6}(\cdot)\) in place of \(\psi(\cdot)\) to generate the approximate policy \(\mutrunc(\cdot)\). We skipped the Lipschitz extension procedure for this example due to minor error fluctuations in the boundary of the feasible set. Figure \eqref{fig:can_Actual_Approx_NMPC} shows the actual and the approximated policies along with the error surface. Table \eqref{tab:metadata_ex_nl_2} collects the computation-time and storage requirement data concerning the explicit feedback law. 
% \begin{figure}[ht]
% \includegraphics[width=8cm,height=6cm]{Figures/can_new_error.eps}
% \caption{The absolute error between \(\upopt(\cdot)\) and \(\mutrunc(\cdot)\) for example \eqref{exmp:nmpc_3}.}\label{fig:can_Actual_Approx_NMPC_Error}
% \end{figure}
Figures \eqref{fig:canale_state} and \eqref{fig:canale_control} depict the closed-loop trajectories obtained via applying QuIFS and \cite{Raimondo2012}. Clearly (see the enlarged snippets within the figures) QuIFS performs better than the algorithm established in \cite{Raimondo2012} in terms of closeness to the online RHC trajectories. 
%%% can state traj %%%
\begin{figure}[ht]
\centering
\includegraphics[scale=0.4]{Figures/can_new_x1x2_modified.eps}
\caption{State trajectories for Example \ref{exmp:nmpc_3} generated by QuIFS, the algorithm reported in \cite{Raimondo2012}, and the online receding horizon state trajectories for \(x_0 \Let \begin{pmatrix}2&-2 \end{pmatrix}^{\top}\) for a simulation length \(120\).}\label{fig:canale_state}
\end{figure}
%%% can control traj %%%
\begin{figure}[ht]
\centering
\includegraphics[scale=0.35]{Figures/new_can_u_modified.eps}
\caption{Control trajectories for Example \ref{exmp:nmpc_3} generated by QuIFS, the algorithm reported in \cite{Raimondo2012}, and the online receding horizon control trajectory for a simulation length \(120\).}\label{fig:canale_control}
\end{figure}
\begin{table}[]
  \centering
\begin{tabular}{lccc}
\toprule
Method  & \textbf{CT} \(\bigl(\mutrunc(\cdot)\bigr)\) & \textbf{CT} (online) & Storage 
\\ \midrule
QuIFS & 51 sec & 0.8 m.sec & 35 KB   \\
\cite{Raimondo2012} &  45 sec & 0.8 m.sec & 28 KB 
\\ \bottomrule
    \end{tabular}
    \caption{Computation-time \textbf{CT} and storage requirement with \(\eps=0.05\) for Example \ref{exmp:nmpc_3}.}
  \label{tab:metadata_ex_nl_2}
\end{table}
\end{example}

